Sigma 1 of PL-homeomorphism groups

I survey the known results about the invariant Sigma 1 of groups of PL-homeomorphisms of a compact interval and supplement them with new results about Sigma 1 of PL-homeomorphism groups of a half line or a line. The proofs are based on the Cayley-graph definition of the invariant.

==> Definitions.tex <==
%
\makeatletter
%
%
\DeclareMathOperator{\ab}{ab}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\Aff}{Aff}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Att}{Att}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Autfr}{\mathfrak{Aut}}
%   B
\DeclareMathOperator{\BPL}{BPL}
%   C
\DeclareMathOperator{\can}{can}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\core}{core}
\DeclareMathOperator{\cpl}{cpl}
%   D
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\Dr}{Dr}
%   E
\DeclareMathOperator{\edg}{edg}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Endfr}{\mathfrak{End}}
\DeclareMathOperator{\exo}{exo}

\DeclareMathOperator{\Ext}{Ext}
%   F
\DeclareMathOperator{\face}{face}
\DeclareMathOperator{\FF}{FF}
\DeclareMathOperator{\Fit}{Fit}
\DeclareMathOperator{\FP}{FP}
\DeclareMathOperator{\Frat}{Frat}
%   G
\DeclareMathOperator{\gp}{gp}
\DeclareMathOperator{\GL}{GL}
%   H
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Homeo}{Homeo}
\DeclareMathOperator{\homeo}{homeo}
%  I
\newcommand{\id}{\mathbbm{1}}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Inn}{Inn}
\DeclareMathOperator{\Incl}{incl.}
\DeclareMathOperator{\inner}{inner}
\DeclareMathOperator{\Int}{int}
%  L
\DeclareMathOperator{\lcm}{lcm}
%   M
\DeclareMathOperator{\md}{md}
%  N
\newcommand{\norm}[1]{\| #1\|}
% O
\DeclareMathOperator{\Out}{Out}
\DeclareMathOperator{\Outfr}{\mathfrak{Out}}
\DeclareMathOperator{\Outer}{outer}
%  P
\DeclareMathOperator{\per}{per}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\PLhomeo}{PL-homeo}
%   R
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\rk}{rk}
%    S
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\St}{St}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\SUPP}{SUPP}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\Sym}{Sym}
%  T
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\TPL}{TPL}
\DeclareMathOperator{\tr}{tr}
%   V
\DeclareMathOperator{\Val}{Val}
\DeclareMathOperator{\ver}{ver}
%


%
%% blackboard letters
%%
\def\B{\mathbb{B}} 
\def\C{\mathbb{C}}
\def\F{\mathbb{F}}
\def\H{\mathbb{H}}
\def\K{\mathbb{K}}
\def\M{\mathbb{M}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\s{\mathbb{S}}
\def\U{\mathbb{U}}
\def\Z{\mathbb{Z}}
%
%
%% Calligraphic letters
\let\@@angstroem=\AA    
\let\angstroem=\@@angstroem
\def\AA{\mathcal{A}}
\def\BB{\mathcal{B}}
\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}
\def\EE{\mathcal{E}}
\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}
\def\HH{\mathcal{H}}
\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}
\def\KK{\mathcal{K}}
\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}
\def\NN{\mathcal{N}}
\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}
\def\QQ{\mathcal{Q}}
\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}
\def\TT{\mathcal{T}}
\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}
\def\WW{\mathcal{W}}
\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}
\def\ZZ{\mathcal{Z}}
%%
% eufrak
%
\def\Afr{\mathfrak{A}} 
\def\Bfr{\mathfrak{B}} 
\def\Ffr{\mathfrak{F}} 
\def\pfr{\mathfrak{p}} 
\def\Sfr{\mathfrak{S}} 
\def\Tfr{\mathfrak{T}} 

% morphisms
\newcommand{\mono}{\rightarrowtail}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\isoinv}{\stackrel{\sim}{\longleftarrow}}
%
% useful abbreviations (see LaTeX Companion, page 80)
%\newcommand{\cf}{cf. \xspace}
\newcommand{\eg}{e.g., \xspace}
\newcommand{\ie}{i.e., \xspace}
\newcommand{\etc}{etc. \@\xspace}
%
% command for left conjugation
%
\newcommand{\act}[1]{\,^{#1}}
%
%
%% Initializing
\setlength{\parindent}{1em}
%
\makeatother
\endinput

==> Old-proof.tex <==
%=========
\section{Proof of Theorem \ref{thm:Generalization-of-BNS-Theorem-8.1} for infinitely generated groups}
\label{sec:Proof-of-first-main-theorem-for-infinitely-generated-groups}
%=========
%
We shall distinguish three cases.
%---------------------
\subsection{Case where $\sigma_\ell$ and $\sigma_r$ are both zero} 
\label{ssec:Case-sigma_ell-rho-trivial}
%---------------------
In this case the group $G$ coincides with $\ker \sigma_\ell$ and also with $\ker \sigma_r$
and so the claim is covered by
%
\begin{prp}
\label{prp:Sigma1-for-bounded-subgroups}
%
Assume $G$ is an irreducible group.
If $\sigma_\ell$ and $\sigma_r$ are trivial then $\Sigma^1(G) = S(G)$.
\end{prp}
\begin{proof}
Given a non-zero character $\chi$ of $G$,
pick an element $h_0 \in G$ with $\chi(h_0) \neq 0$ 
and consider the set $J$ of its conjugates in $G$.
Since $G$ is irreducible and $h_0$ is the identity near the endpoints of the interval $I$, 
the set $J$ enjoys then the following properties:
\begin{enumerate}[a)]
\item for every pair of elements $h_1$ and $h_2$ in  $J$ 
there exists $h_3 \in J$ that centralizes both $h_1$ and $h_2$;
%
\item for every $g \in G$ there exists $h \in J$ that centralizes $g$.
\end{enumerate}
Assume now that $G$ acts on a measured tree with associated character $\chi$.
\footnote{See \cite[Section C2.4]{Str13a} for the notions of measured tree and of hyperbolic element.
Alternatively, one could work with abelian $(G,\R)$-trees in the sense of \cite[Section 1]{Bro87b}.}
Every element of  $h \in J$ is hyperbolic and so it has an axis $A_h$;
in view of property a) these axes coincide (see \cite[Lemma C2.23]{Str13a}).
Property b) then implies that this common axis $A$ in mapped onto itself 
by every element of $G$ and so the axis $A$ is $G$-invariant. 
As this conclusion holds for every measured $G$-tree,
$[\chi] \in \Sigma^1(G)$ by Theorem C2.35 in \cite{Str13a}
 (actually, only the easy implication $(ii) \Rightarrow (i)$ of this theorem is needed).
 \end{proof}
 
 %---------------------
\subsection{Case where exactly one of $\sigma_\ell$ and $\sigma_r$ is zero} 
\label{ssec:Case-one-of-sigma_ell-rho-is-trivial}
%---------------------
Suppose first that $\sigma_\ell$ is not zero, but $\sigma_r$ is trivial.
Then $G/\ker \chi_r$ is the trivial group;
as $G$ is irreducible it is therefore non-abelian by Lemma \ref{lem:G-non-abelian}
and so $[\chi_\ell] \in \Sigma^1(G)^c$ by Proposition \ref{prp:Roles-of-chi-ell-and-chi-r}.

Suppose now that $\chi$ is a non-zero character  
that does not represent $[\chi_\ell]$.
Condition (i) of Lemma \ref{lem:Existence-elements-f-and-h} is then satisfied
and so there exist elements $f$, $h$ in $G$ 
and a positive real number $\delta$ with these properties:
\begin{align}
\chi(f) > 0,& \quad f \text{ is linear on } [a,a+ \delta] \text{ with slope } < 1,
\label{eq:Property-f}\\
%
\chi(h) > 0,& \quad \supp h \subset [a, a+\delta].
\label{eq:Property-h}
\end{align}
%
Consider now a finite subset $\XX_1$ of $G$ that includes both $f$ and $h$
and let $G_1$ denote the subgroup generated by $\XX_1$.
For every commutator $c$ in $G$ there exists then a positive integer $m$ 
so that the supports of $\act{f^m}h$ and $c$ are disjoints,
and so it follows, 
as in the proof of Lemma \ref{lem:Sufficient-condition-for-point-in-Sigma1},
that $\chi \restriction{G_1}$ represents a point of $\Sigma^1(G_1)$.
The group $G$ itself  is the union of such finitely generated subgroups $G_1$;
as $\chi$ does not vanish on the intersection of two such subgroups
(for both contain the elements $f$ and $h$)
Proposition \ref{prp:Membership-for-infinitey-generated-groups}
allows us to conclude
that  $[\chi] \in \Sigma^1(G)$.

The case where  $\sigma_\ell$ is zero, but $\sigma_r$ is not, can be handled similarly.
 

%---------------------
\subsection{Case where $\sigma_\ell$ and $\sigma_r$ are non-zero} 
\label{ssec:Case-both-sigma_ell-sigma_r-non-trivial}
%---------------------
By assumption,
 $G/(\ker \sigma_\ell \cdot \ker \sigma_r)$ is a torsion group;
since $G$ is irreducible it is therefore non-abelian by Lemma \ref{lem:G-non-abelian}.
Proposition \ref{prp:Roles-of-chi-ell-and-chi-r} thus implies
that $\chi_\ell$ and $\chi_r$ represent points outside of $\Sigma^1(G)$.
 
Suppose now that $[\chi]$ is a non-zero character 
and  that  $[\chi] \neq [\chi_\ell]$ and $[\chi] \neq [\chi_r]$.
The image of $\chi$ is then an infinite subgroup of $\R$;
as $G/(\ker \chi_\ell \cdot \ker_r)$ is a torsion group,
the character $\chi$ does therefore not vanish on $\ker \chi_\ell \cdot \ker \chi_r$
and so at least one of $\chi(\ker \sigma_r)$ or $\chi(\ker \sigma_\ell)$ is non-zero.
Assume first that $\chi (\ker \sigma_r) \neq \{0\}$.
Then condition (i) of Lemma \ref{lem:Existence-elements-f-and-h} holds
and so the lemma provides one with elements $f$, $h$ of $G$ 
and a real number $\delta$ that enjoy certain properties.
These properties allow one to deduce, 
exactly as in the proof given in section \ref{ssec:Case-one-of-sigma_ell-rho-is-trivial},
that $[\chi] \in \Sigma^1(G)$.
If, on the other hand, 
$\chi$ does not vanish on $\ker \sigma_\ell$
then condition (ii) of Lemma \ref{lem:Existence-elements-f-and-h} is satisfied,
whence one finds, as before,  elements $f$, $h$ of $G$ 
and a real number $\delta$ with certain properties
(see equation \eqref{eq:Consequence-ii} for more details).
They allow one to infer that $[\chi] \in \Sigma^1(G)$.

